Hopper: Bounded-Memory Collaborative Debiasing for Byzantine-Tolerant Peer Sampling

Byzantine-tolerant peer sampling relies on continuously refreshed views, yet an adversary can bias the identifier streams used to construct them. Frequency-aware debiasing downweights overrepresented identifiers, but existing designs rely on cumulative per-identifier counts. We show that even exact, unbounded counters fail under a delayed balanced attack, in which a long benign prefix masks a subsequent adversarial frequency shift. We introduce Hopper, a bounded-memory debiasing protocol for Byzantine-tolerant peer sampling. We identify the stream-estimation properties required for debiasing and select BitMatcher as the estimator that best preserves adversarial frequency structure among the evaluated alternatives. Hopper adds BMDecay, a saturation-triggered decay and reconstruction mechanism that keeps this signal fresh over long executions. Hopper also supports trusted collaboration through authenticated fingerprint-aware reconstruction and role-specific debiasing. Experiments show that Hopper recovers from delayed attacks faster than when relying on BitMatcher, and debiaising as well as non-debiasing baselines under a fixed memory budget. Trusted collaboration reduces post-attack pollution peaks but creates a re-identification trade-off at high trusted-node densities. These results show the importance of occurence freshness, rather than exact counting alone, as a key requirement for practical frequency-aware Byzantine peer sampling.

==> sections/eval_robust_estim.tex <==
\section{Estimator Selection}
\label{sec:estimator-eval}

We now determine which fixed-budget estimator best preserves the information Hopper needs.
The objective is adversarial debiasing, not generic average estimation error.
All experiments in this section are single-node microbenchmarks: one estimator consumes a generated identifier stream and is queried after ingestion.
Protocol behavior is evaluated separately in Section~\ref{sec:bmdecay-eval}.





We retained estimators with bounded $B$-byte memory and inexpensive operations and identify representation-specific risks (Table~\ref{tab:sketches}) before evaluating benign and adversarial streams under various parameters that stress the estimator's quality in peer sampling contexts, \ie, various memory budget, stream length, and population size.




\subsection{Method}
\label{sec:estimator-setup}

We generate streams inspired by the scale of Bitcoin peer discovery: \(N=20{,}000\) identifiers and \(M=600{,}000\) to \(7.2\) million observations, corresponding approximately to 30 days through one year at 20,000 received identifiers per day~\cite{bitnode:07072025}.
An exact array of four-byte counters requires 80 KB; sketch budgets range from 20 to 80 KB.
Uniform streams sample all identifiers equally.
Adversarial streams use Byzantine fractions \(f\in\{10\%,20\%,30\%\}\) and bias factor \(\gamma=10\); Figure~\ref{fig:input-streams} shows the resulting two-class distribution.
Every Byzantine identifier receives weight \(\gamma\), every correct identifier weight one, and observations are drawn from the normalized population.
This isolates balanced-attack frequency structure rather than modeling packet-level behavior.

\begin{figure}[!t]
  \centering
  \includegraphics[width=.48\linewidth]{figures/sketch/stream20000-600000-20-10-20-matplotlib.pdf}
  \caption{Identifier distribution N=20K, M=600K, f=20\%, $\gamma$=10}
  \label{fig:input-streams}
\end{figure}

We evaluate BitMatcher (BM), Cold Filter (CF), Count-Min Sketch with Conservative Updates (CMSCU), Count-Mean-Min with Conservative Updates (CMMCU), Lossy Conservative Update (LCU), and XY.
Count-Min variants use three hash functions; Cold Filter assigns 90\% of memory to filtering layers and 10\% to its CMSCU backing sketch~\cite{goyal:2012,coldfilter:2019}.
For each stream, we query every identifier and compute the metrics from Section~\ref{sec:estimator-properties}.
We vary one pressure source at a time: memory budget at fixed \(N\) and \(M\), stream length at fixed \(N\) and budget, and population size at fixed \(M\) and budget.

\subsection{Results and Selection}
\label{sec:adversarial-sketch-results}

In uniform streams, CMSCU and Cold Filter obtain near-zero KL divergence; BitMatcher becomes more sensitive as memory per identifier decreases.
This sanity check does not determine suitability under attack: Hopper's decision depends on preserving frequency contrast.
BitMatcher's advantage is thus specific to adversarial skew, not generic frequency estimation.

Under adversarial bias, BitMatcher consistently best preserves the relevant structure.
Figure~\ref{fig:sketch-budget} varies memory at \(M=600{,}000\).
BM obtains the lowest KL divergence, maintains high \(F_1\), and keeps bias-factor error near zero across Byzantine fractions.
Most alternatives underestimate \(\gamma\), which would admit Byzantine identifiers too often.
Collision and correction errors in the alternatives reduce the measured contrast between classes.

\begin{figure}[!t]
  \centering
  \includegraphics[width=\linewidth]{figures/sketch/dKL_on_budget_20000-600000-10-legend.pdf}
  \includegraphics[width=\linewidth]{figures/sketch/f1score_on_budget_20000-600000-10.pdf}
  \includegraphics[width=\linewidth]{figures/sketch/cratio_on_budget_20000-600000-10.pdf}
  \caption{Estimator quality versus memory: KL divergence, \(F_1\), and bias-factor error. Columns show \(f=10\%,20\%,30\%\).}
  \label{fig:sketch-budget}
\end{figure}

Figure~\ref{fig:sketch-stream} varies stream length at 40 KB.
BM remains best, but gradually loses capacity and bias-factor accuracy; thus standard BitMatcher cannot support an unbounded execution unchanged.
Large counters continue to represent hot identifiers while the estimator increasingly fails to retain new or cold fingerprints, motivating capacity-reclaiming aging.

\begin{figure}[!t]
  \centering
  \includegraphics[width=\linewidth]{figures/sketch/dKL_on_stream_20000-40KB-10.pdf}
  \includegraphics[width=\linewidth]{figures/sketch/f1score_on_stream_20000-40KB-10.pdf}
  \includegraphics[width=\linewidth]{figures/sketch/cratio_on_stream_20000-40KB-10-legend.pdf}
  \caption{Estimator quality versus stream length at 40 KB. Columns show \(f=10\%,20\%,30\%\).}
  \label{fig:sketch-stream}
\end{figure}

Increasing \(N\) at fixed memory produces similar pressure (Figure~\ref{fig:sketch-n}).
BM still best preserves the bias factor, although fingerprint collisions reduce class precision.

\begin{figure}[!t]
  \centering
  \includegraphics[width=\linewidth]{figures/sketch/dKL_on_nodes_600000-40KB-10.pdf}
  \includegraphics[width=\linewidth]{figures/sketch/f1score_on_nodes_600000-40KB-10.pdf}
  \includegraphics[width=\linewidth]{figures/sketch/cratio_on_nodes_600000-40KB-10-legend.pdf}
  \caption{Estimator quality versus population size at 40 KB. Columns show \(f=10\%,20\%,30\%\).}
  \label{fig:sketch-n}
\end{figure}

We therefore select BitMatcher for Hopper.
Its bounded-stream accuracy satisfies the debiasing objective; its saturation and non-linear representation are handled by Hopper-D and Hopper's trusted merge, respectively.

